Flexible Dynamic Information Flow Control in the Presence of Exceptions

We describe a new, dynamic, floating-label approach to language-based information flow control. A labeled IO monad, LIO, keeps track of a current label and permits restricted access to IO functionality. The current label floats to exceed the labels of all data observed and restricts what can be modified. Unlike other language-based work, LIO also bounds the current label with a current clearance that provides a form of discretionary access control. Computations may encapsulate and pass around the results of computations with different labels. In addition, the LIO monad offers a simple form of labeled mutable references and exception handling. We give precise semantics and prove confidentiality and integrity properties of a call-by-name \lambda-calculus and provide an implementation in Haskell.

==> GNUmakefile <==
MAIN = main.ltx
PDF = pdf

ifeq ($(PDF),pdf)
FIGEXT    = pdf
OUTEXT    = pdf
else
FIGEXT    = eps
OUTEXT    = dvi
endif

BASE      := $(basename $(MAIN))
SRCEXT    := $(patsubst $(BASE).%,%,$(MAIN))
XFIGS     := $(wildcard *.fig)
DIAFIGS   := $(wildcard *.dia)
SVGFIGS   := $(wildcard *.svg)
TEXFIGS   := $(XFIGS:.fig=.tex) # $(DIAFIGS:.dia=.tex)
BINFIGS   := $(XFIGS:.fig=.$(FIGEXT)) $(DIAFIGS:.dia=.$(FIGEXT)) $(SVGFIGS:.svg=.$(FIGEXT)) $(GENFIGS)
STYLINK	  := $(notdir $(wildcard ../*.sty))
STYFILES  := $(sort $(STYLINK) $(wildcard *.sty))
TEXFILES  := $(sort $(MAIN) $(wildcard *.tex) $(STYFILES) $(TEXFIGS))
BIBFILES  := $(wildcard *.bib)

JGRAPHS   := $(wildcard *.j)
GGRAPHS   := $(wildcard *.gnuplot)
GRAPHS    := $(JGRAPHS.j=.$(FIGEXT)) $(GGRAPHS:.gnuplot=.$(FIGEXT))

ifeq ($(PDF),pdf)
IMAGESRC  := $(wildcard figs/*.gif) $(wildcard figs/*.eps) 
else
IMAGESRC  := $(wildcard figs/*.gif) 
endif
IMAGEGEN  := $(addsuffix .$(FIGEXT), $(basename $(IMAGESRC)))
IMAGES    := $(sort $(IMAGEGEN) $(wildcard figs/*.$(FIGEXT)))
IMAGEDIST := $(filter-out $(IMAGEGEN), $(IMAGES)) \
		$(wildcard figs/*.odp) $(wildcard figs/*.ppt)

ifeq ($(PDF),pdf)
LATEX     = pdflatex \\nonstopmode\\input
else
LATEX     = latex
#\\nonstopmode\\input
DVIPS     = dvips -j0 -G0 -t letter -Pdownload35
PS2PDF    = GS_OPTIONS=-sPAPERSIZE=letter ps2pdf -sPAPERSIZE=letter -dEmbedAllFonts=true
#PS2PDF    = ps2pdf
endif
BIBTEX    = bibtex -min-crossrefs=1000

all: $(BASE).pdf

ifeq ($(PDF),pdf)
%.pdf %.tex: %.fig
	fig2dev -L pdftex -p1 $< > $*.pdf
	fig2dev -L pdftex_t -p $*.pdf $< > $*.tex

%.pdf: %.eps
	perl -ne 'exit 1 unless /\n/' $< \
		|| perl -p -i -e 's/\r/\n/g' $<
	epstopdf --outfile=$@ $<

figs/%.pdf: figs/%.gif
	convert $< $@

%.ps: %.pdf
	pdftops -paper A4 $< $@

else
%.ps: %.dvi
	$(DVIPS) $< -o $@

%.eps %.tex: %.fig
	fig2dev -L pstex -p1 $< > $*.eps
	fig2dev -L pstex_t -p $*.eps $< > $*.tex
endif

%.eps: %.dia
	unset DISPLAY; dia -n -e $@ $<
%.tex: %.dia
	unset DISPLAY; dia -n -e $@ $<
%.eps: %.j
	@rm -f $@~
	jgraph $< > $@~
	mv -f $@~ $@
%.eps: %.gnuplot %.data
	gnuplot $*.gnuplot
%.pdf: %.svg
	inkscape -z -A $@ $< && cp $@ .missing/$@ || cp .missing/$@ $@

$(STYLINK):
	rm -f $@
	ln -s ../$@ .

RERUN = egrep -q '(^LaTeX Warning:|\(natbib\)).* Rerun' $*.log
UNDEFINED = egrep -q '^(LaTeX|Package natbib) Warning:.* undefined' $*.log

# So you can "setenv ALWAYS yes" instead of butchering the Makefile...
ifneq ($(ALWAYS),)
ALWAYS = always
endif
$(BASE).$(OUTEXT): %.$(OUTEXT): %.$(SRCEXT) $(TEXFILES) $(BIBFILES) \
				$(BINFIGS) $(GRAPHS) $(IMAGES) $(ALWAYS)
	test ! -s $*.aux || $(BIBTEX) $* || rm -f $*.aux $*.bbl
	$(LATEX) $< || ! rm -f $@
	if $(UNDEFINED); then \
		$(BIBTEX) $* && $(LATEX) $< || ! rm -f $*.bbl $@; \
	fi
	! $(RERUN) || $(LATEX) $< || ! rm -f $@
	! $(RERUN) || $(LATEX) $< || ! rm -f $@
ifeq ($(PDF),pdf)
	touch $*.dvi
	test ! -f .xpdf-running || xpdf -remote $(BASE)-server -reload
else
$(BASE).pdf: %.pdf: %.ps
	$(PS2PDF) $< $@
	test ! -f .xpdf-running || xpdf -remote $(BASE)-server -reload
endif

DIST = GNUmakefile $(filter-out $(TEXFIGS), $(TEXFILES)) \
	$(XFIGS) $(DIAFIGS) $(SVGFIGS) $(GENFIGSRC) \
	$(JGRAPHS) $(GGRAPHS) $(GGRAPHS:.gnuplot=:.data) \
	$(IMAGESRC) $(IMAGEDIST) $(BIBFILES)
dist: $(BASE).tar.gz
$(BASE).tar.gz: $(DIST)
	tar -chzf $@ -C .. \
		$(patsubst %, $(notdir $(PWD))/%, $(DIST))

PREVIEW := $(BASE)
preview: $(PREVIEW).pdf
	if test -f .xpdf-running; then			\
		xpdf -remote $(BASE)-server -quit;	\
		sleep 1;				\
	fi
	touch .xpdf-running
	(xpdf -remote $(BASE)-server $(PREVIEW).pdf; rm -f .xpdf-running) &

show: $(BASE).pdf
	xpdf -fullscreen $(BASE).pdf

osx: $(BASE).pdf
	open $(BASE).pdf

check:
	pdflatex $(BASE).ltx | grep -e "multiply" -e "undefined"

EXTRAIGNORE = '*~' '*.aux' '*.bbl' '*.blg' '*.log' '*.dvi' '*.bak' '*.out'
ignore:
	rm -f .gitignore
	(for file in $(EXTRAIGNORE); do \
		echo "$$file"; \
	done; \
	for file in .xpdf-running \
			$(BASE).tar.gz \
			$(TEXFIGS) $(BINFIGS) $(GRAPHS) $(IMAGEGEN) \
			$(BASE).ps $(BASE).pdf; do \
		echo "/$$file"; \
	done) | sort > .gitignore
	git add .gitignore

clean:
	rm -f $(BASE).ps $(BASE).pdf $(BASE).tar.gz
	rm -f $(TEXFIGS) $(GRAPHS) $(IMAGEGEN)
	rm -f *.dvi *.aux *.log *.blg *.lof *.lot *.toc *.bak *.out
	rm -f *~ *.core core

binfigsclean: clean
	rm -f $(BINFIGS)

always:
	@:

.PHONY: install clean binfigsclean all always ignore preview show osx dist

spell:
	make clean
	for i in $(wildcard *.tex); do aspell -p ./aspell.words -c $$i; done

flat:
	./flatten.pl $(MAIN) > $(BASE)-flat.tex

proof:
	./weasel *.tex
	./passive *.tex


==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

We propose a new design point for IFC systems in which most
values in lexical scope are protected by a single, mutable,
\emph{current label}, yet one can also encapsulate and pass around
the results of computations with different labels.  
Unlike other language-based work, our
model provides a notion of \emph{clearance} that imposes
an upper bound on the program label, thus providing
a form of discretionary access control on portions
of the code.

We prove information flow and integrity properties of
our design and describe LIO, an implementation of the new model in Haskell.
LIO, which can be implemented entirely as a library,
demonstrates both the applicability and simplicity of the approach.
We show the capabilities of the library to perform secure side-effects (e.g., references) 
as well as safely handle exceptions. 
Our non-interference theorem proves the conventional property that
lower-level results do not depend on higher-level inputs --
the label system prevents inappropriate flow of information.
We also prove confinement theorems that show the effect of
clearance on the behavior of code.
In effect, lowering the clearance imposes a discretionary
form of access control by preventing subsequent code (within 
that scope) from accessing higher-level information.

As an illustration of the benefits and expressive power
of this system, we describe a reviewing system that uses
LIO labels to manage integrity and confidentiality
in an environment where users and labels are added dynamically. 
Although we have use LIO for the \review{} API and 
even built a relatively large web-framework that securely
integrates untrusted third-party applications, we believe that
changes in the constructs are likely to occur as the language
matures. This further supports our library-based approach to
language-based security.

%% An interesting future work consists on extending our library to handle 
%% concurrency. Enforcement mechanisms for
%% sequential programs do not generalize naturally to 
%% multithreaded programs. 
%% In this light, it is hardly surprising that Jif~\cite{myers:jif},
%% the mainstream IFC compiler, lack support 
%% for multithreading. Due to the monadic structure of LIO programs, 
%% we believe it is possible to extend our library to consider concurrency
%% that also addresses termination~\cite{askarov:termination-insensitive} 
%% and internal-timing leaks~\cite{Volpano:Smith:Probabilistic}.

% Local Variables:
% reftex-bibpath-environment-variables: "./"
% TeX-master: "main.ltx"
% tex-main-file: "main.ltx"
% tex-command: "gmake;:"
% tex-dvi-view-command: "gmake preview;:"
% End:


==> notation.tex <==
\newcommand{\ssin}{\ensuremath{\tilde{\upepsilon}}}
\newcommand{\lang}{\ensuremath{\lambda^\to_{\ell}}}
\newcommand{\review}{\ensuremath{\lambda\textrm{Chair}}}
%\newcommand{\implies}{\Rightarrow}
\newcommand{\Coloneqq}{::=} % txfonts
\newcommand{\dom}{\ensuremath{{\textrm{dom}}}}
\newcommand{\Lcurr}{\ensuremath{L_{\textrm{cur}}}}
\newcommand{\Ccurr}{\ensuremath{C_{\textrm{cur}}}}

% terms:
\newcommand{\LrName}{\texttt{Lb}}
\newcommand{\Lr}[2]{\LrName\ #1\ #2}
\newcommand{\lioValp}[1]{(#1)^\texttt{\tiny LIO}}
\newcommand{\true}{\texttt{true}}
\newcommand{\false}{\texttt{false}}
\newcommand{\unit}{\texttt{()}}
\newcommand{\fix}[1]{\texttt{fix}\ #1}
\newcommand{\proj}[2]{\pi_{#1}\ #2}
\newcommand{\ifel}[3]{\texttt{if}\ #1\ \texttt{then}\ #2\ \texttt{else}\ #3}
\newcommand{\letbind}[3]{\texttt{let}\ #1=#2\ \texttt{in}\ #3}
\newcommand{\withLblClr}[2]{\texttt{withLblClr}\ #1\ #2}
\newcommand{\lowerClr}[1]{\texttt{lowerClr}\ #1}
\newcommand{\lowerClrName}{\texttt{lowerClr}}
\newcommand{\lref}[2]{\lrefName\ #1\ #2}
\newcommand{\openR}[1]{\openRName\ #1}
\newcommand{\closeR}[2]{\closeRName\ #1\ #2}
\newcommand{\lrefName}{\texttt{label}}
\newcommand{\openRName}{\texttt{unlabel}}
\newcommand{\closeRName}{\texttt{toLabeled}}

\newcommand{\rulefont}[1]{\textsc{#1}}
\newcommand{\pc}{\texttt{pc}}

\newcommand{\returnLIOp}[1]{\returnLIOpName \ #1}
\newcommand{\bindLIOp}[2]{#1\ \bindLIOpName \ #2}
\newcommand{\returnLIOpName}{\texttt{return}}
\newcommand{\bindLIOpName}{\texttt{>>=}}
\newcommand{\newRef}[2]{\newRefName\ #1\ #2}
\newcommand{\readRef}[1]{\readRefName\ #1}
\newcommand{\writeRef}[2]{\writeRefName\ #1\ #2}
\newcommand{\newRefName}{\texttt{newLIORef}}
\newcommand{\readRefName}{\texttt{readLIORef}}
\newcommand{\writeRefName}{\texttt{writeLIORef}}
\newcommand{\labelOfR}[1]{\texttt{labelOf}\ #1}
\newcommand{\labelOfRef}[1]{\texttt{labelOfRef}\ #1}
\newcommand{\curLbl}{\texttt{getLabel}}
\newcommand{\curClr}{\texttt{getClearance}}

% types:
\newcommand{\LrefName}{\texttt{Labeled}}
\newcommand{\Lref}[2]{\LrefName \ #1\ #2}
\newcommand{\LIOName}{\texttt{LIO}}
\newcommand{\LIOp}[2]{\LIOName\ #1\ #2}
\newcommand{\Ref}[2]{\texttt{Ref}\ #1\ #2}
\newcommand{\Bool}{\texttt{Bool}}

% environment related:
\newcommand{\env}{\Sigma}
\newcommand{\wEnv}[2]{\langle #1, #2 \rangle}
\newcommand{\defEnv}[1]{\wEnv{\env}{#1}}
\newcommand{\store}{\phi}
\newcommand{\lbl}{\texttt{lbl}}
\newcommand{\clr}{\texttt{clr}}

% label related:
\newcommand{\flows}{\sqsubseteq}
\newcommand{\lub}{\sqcup}
\newcommand{\glb}{\sqcap}
\newcommand{\lpure}{l_\bot}
\newcommand{\lclear}{l_\top}
\newcommand{\nolabel}{\obslash}

% exception related
\newcommand{\Exception}{\mathbf{X}}
\newcommand{\throwName}{\texttt{throwLIO}}
\newcommand{\throw}[1]{\throwName\ {#1}}
\newcommand{\catchName}{\texttt{catch}}
\newcommand{\catch}[2]{\catchName\ #1\ #2}



% arrows
\newcommand{\lto}{\longrightarrow}

% term erasure
\newcommand{\hole}{\bullet}
\newcommand{\eraseName}{\varepsilon}
\newcommand{\erase}[2]{\eraseName_{#1}(#2)}
\newcommand{\el}[1]{\erase{L}{#1}}
\newcommand{\mkEnt}[2]{$\el{#1}=#2$}
\newcommand{\mkEntTwo}[2]{\el{#1}=#2}

% simple lattice
\newcommand{\lL}{\texttt{L}}
\newcommand{\lM}{\texttt{M}}
\newcommand{\lH}{\texttt{H}}
\newcommand{\lE}{\texttt{E}}


% relational:
\newcommand{\rnv}{\mathcal{R}}
\newcommand{\dbInsert}[1]{\texttt{insert}\ #1}
\newcommand{\dbQuery}[2]{\texttt{query}\ #1\ #2}
\newcommand{\dbUpdate}[2]{\texttt{update}\ #1\ #2}
\newcommand{\dbDelete}[1]{\texttt{delete}\ #1}
\newcommand{\dbSel}[2]{\texttt{sel}\ #1\ #2}

\newcommand{\wRnv}[3]{\langle #1;#2, #3 \rangle}
\newcommand{\defRnv}[1]{\wRnv{\env}{\rnv}{#1}}
\newcommand{\rlbl}{\texttt{rlbl}}
\newcommand{\rclr}{\texttt{rclr}}

% DCLabels
\newcommand{\dcL}[2]{\left\langle\left\{#1\right\}, \left\{#2\right\}\right\rangle} 
\newcommand{\dcLL}[2]{\left\langle  #1, \ #2 \right\rangle} 
\newcommand{\CFL}{\texttt{\#CONFLICT}}

% proof helpers
%\newcommand{\remove}[3]{\left(#3\right)_{\downarrow #1}^{\uparrow #2}}
\newcommand{\removeLbl}[2]{(#2)_{\downarrow #1}}
\newcommand{\removeClr}[2]{(#2)_{\uparrow #1}}
\newcommand{\nrToLabeled}[1]{\#(#1)}


==> related.tex <==
\section{Related Work}\label{sec:related}

Heintze and Riecke~\cite{Heintze:Riecke:Slam} 
consider security for lambda-calculus where 
lambda-terms are explicitly annotated with security labels,
for a type-system that guarantees non-interference.
\cut{
One of the key aspects of this work consists on the 
operator $\mathbf{protect_{ir}~ e}$, which raises the security annotation of $e$ to, at least, $ir$.
Similarly, our approach raises the current label in the state of the $\LIOp$ monad when manipulating 
labeled values. 
}
One of the key aspects of their work consists of an operator which raises the
security annotation of a term in a similar manner to our raise of the current
label when manipulating labeled values.
%
% floating labels
Similar ideas of floating labels have been used by many operating systems,
dating back to the High-Water-Mark security model~\cite{landwehr:formal-models} of
the ADEPT-50 in the late 1960s.
Asbestos~\cite{efstathopoulos:asbestos} first combined floating labels
with the Decentralized label model~\cite{myers:dlm}.


%% DCC
Abadi et al. \cite{Abadi+:Core} develop the dependency core calculus (DCC)
 based on a hierarchy of monads to guarantee
non-interference. In their calculus, they define a %the type $T_\ell(s)$ 
monadic type that ``protects'' (the confidentiality of) side-effect-free
values at different security levels.
Though not a monad, our $\LrefName$ type similarly protects pure values at
various security levels.
To manipulate such values, DCC uses a non-standard
typing rule for the bind operator; the essence of this operator, in a
dynamic setting with side-effectful computations, is captured in our library
through the interaction of of $\LrefName$, $\openRName$, and $\LIOName$.
\cut{
Intuitively, 
given $e$ of type $T_\ell(s)$, the resulting type for 
$\mathtt{bind}~x=e~\mathtt{in}~e'$ consists on a type 
$t$, not necessarily $T_\ell$, that is ``protected'' by $\ell$. 
A type $t$ is protected by $\ell$ if the type 
denotes a value with confidentiality level, at least, $\ell$. 
For instance, 
the type $(T_{\ell_1} (\mathtt{Int}), T_{\ell_2} (\mathtt{Int}) )$ 
is protected by $\ell$ if $\ell \sqsubseteq \ell_1$ and 
$\ell \sqsubseteq \ell_2$.
However,
when manipulating 
values of type $\Lref{\ell}{\tau}$ inside 
an $\LIOp$ computation (recall function $\openRName$), 
the \emph{current label} is raised, at least, to the 
security level $\ell$; and thus 
``protecting'' the result of the $\LIOp$ computation 
by $\ell$. In other words,
 the interaction of $\Lref{\ell}{\tau}$, $\openRName$, 
and $\LIOp$ captures the essence of the DCC's
$\mathtt{bind}$ operator for a dynamic setting with 
side-effectful computations.
}

%% DCC into system F
Tse and Zdancewic  \cite{Tse:Zdancewic:ICFP04} translate
DCC to System F and show that non-interference can be stated
using the parametricity theorem for System F.
The authors also provide a Haskell implementation for a two-point
lattice. Their implementation encodes each security level as an abstract data type constructed from functions and binding 
operations to compose computations with permitted flows. 
Since they consider the same non-standard features for 
the $\mathtt{bind}$ operation as in DCC, they 
provide as many definitions for $\mathtt{bind}$ as different 
type of values produced by it. 
Moreover, their implementation needs to be 
compiled with the flag 
\texttt{-fallow-undecidable-instances}, in GHC. Our work, in contrast, defines
only one bind operation for $\LIOName$, without the need for such compiler extensions.
 
% Separation kernels
Harrison and Hook show how to implement an abstract 
operating system called \emph{separation kernel} 
\cite{Harrison05}.
Programs running under this multi-threading operating system 
satisfy non-interference. To achieve this, the authors rely 
on the state monad to represent threads, monad transformers 
to present parallel composition, and the resumption 
monad to achieve communication between threads. 
Consequently, non-interference is enforced by the
scheduler implementation, which only allow signaling threads at
the same, or higher, security level as the thread that issued the 
signal. The authors use monads differently from us;
their goal is to construct secure kernels rather than provide
information-flow security as a library.
\cut{
For instance, we do not use the resumption monad since we do not model threads. 
As a result, our library is simpler and more
suitable to write sequential programs in Haskell. It is stated as a
future work how to extend our library to include concurrency.
}
Our library is simpler and more suitable for writing sequential programs in Haskell.
Extending our library to include concurrency is stated as a future work.

%% Crary et al. 
Crary et al.~\cite{Crary:2005} design a monadic calculus for non-interference for
programs with mutable state. Similar to our work, 
their language distinguishes between term and expressions, where 
terms are pure and expressions are (possibly) effectful computations. 
Their calculus mainly tracks information flow by statically approximating  
the security levels of effects produced by expressions. 
\cut{
Expressions can be included at 
the term level as an element of the monadic type $\bigcirc_{(r,w)} A$, which
denotes a suspended computation where the security level $r$ is an
upper bound on the security levels of the store locations that the
suspended computation reads, while $w$ is a lower bound on the 
security level of the store locations to which it writes. Similarly,  our approach allows expressions to be included at the term level by wrapping them with the constructor $\LrefName$.
}
Compared to their work, we only need to make approximations of the
side-effects of a given computation when using $\closeRName$; the state of
$\LIOp$ keeps track of the dynamic security level upper bound of
observed data. Overall, our dynamic approach is more flexible and permissive
than their proposed type-system.
\cut{
In other words, $\LIOp$ dynamically determines $r$ and forces $r \sqsubseteq w$
for most of the cases.
Thanks to the dynamic nature of $\LIOp$, our approach 
is more flexible and permissive than the type-system proposed by Crary et al.
}



% Authors in-
% troduce the notion of informativeness in order to relax some typ-
% ing rules so that reading and writing into secret store locations can
% be included in large computations related to public data. A type
% A is informative at security level r or above if its values can be
% used or observed by computations that may read data from secu-
% rity level r or above. In our library, the type SecIO s a makes the
% value of type a only informative at security level s. In principle,
% the value of type a cannot be used anywhere but inside the monad
% SecIO s. Considering a two-point lattice, we introduce the func-
% tion plug :: Less L H => SecIO H a -> SecIO L (Sec H
% a) to allow reading and writing secret files into computations re-
% lated to public data. Observe that the function preserves the infor-
% mativeness of a by placing it inside of the monad Sec H.


Pottier and Simonet~\cite{Pottier:Simonet:POPL02,FlowCaml} designed
FlowCaml, a compiler to enforce non-interference for OCaml programs.
%Unfortunately, FlowCaml has not been actively developed since 2003.
Rather than implementing a compiler from scratch, and more similar to our
approach, the seminal work by Li and Zdancewic~\cite{LiZdancewic:CSFW06}
presents an implementation of information-flow security as a library, in
Haskell, using a generalization of monads called
Arrows~\cite{hughes00generalising}.
Extending their work, Tsai et al.~\cite{tsai:multi-threaded-iflow} further
consider side-effects and concurrency.
Contributing to library-based approaches,
Russo et al.~\cite{russo:iflow-haskell} eliminate the need for Arrows by
showing an IFC library based solely on monads.
Their library defines monadic types to track information-flow in
pure and side-effectful computations. Compared to our dynamic IFC library,
Russo et al.'s library is slightly less permissive and leverages Haskell's
type-system to statically enforce non-interference.
However, we note that our library has similar (though dynamic) functions provided by
their SecIO library; similar to $\openRName$, they provide a function
that maps pure labeled values into side-effectful computations; similar to
$\closeRName$, they provide a function that allows reading/writing secret files
into computations related to public data.

\cut{
The library defines monads \hs!Sec s!
and \hs!SecIO s! to respectively track information-flow in pure and
side-effectful computations, where \hs!s! is a security level represented as a singleton type. Russo et al.'s work uses Haskell's type-system to statically
enforce non-interference. In contrast, our library presents a dynamic
enforcement: It is in the execution of $\LIOName$ computations 
where the
non-interference policy is enforced. 
Thanks to that dynamism, our library is more 
permissive than the one proposed by Russo et al~\cite{sabelfeld:dynamic-static}. 
We deliberately choose not to have a monad for securing pure values. Instead, our library manipulates pure values 
inside the $\LIOName$ monad by utilizing the function $\openRName$. 
Similarly, Russo et al.'s work allows this behavior by providing the function \hs!value :: Sec s a -> SecIO s a!, which maps any pure values into side-effectful computations. Considering a two 
point lattice
(\hs!L! for public and \hs!H! for secret data), the function \hs!plug :: SecIO H a -> SecIO L (Sec H a)! %in \cite{russo:iflow-haskell}  
allows reading and writing secret files into computations related to 
public data. To achieve a similar effect as \hs!plug!, our library 
provides the primitive $\closeRName$. 
Additionally, our library represents
security labels as values of a given data type, which facilitates the modeling
of dynamic policies. %, e.g., principals can be added at run-time by %just creating
%new values of such data types. 
Similar to \hs!Sec s! and \hs!SecIO s!, the
correctness of our approach relies on the fact that
attackers are not able to break neither the monadic abstraction provided by $\LIOName$ nor the data abstraction provided by $\LrefName$. Russo et al. briefly
hinted that there are features in Haskell that could allow such
vulnerabilities. We have been recently involved in bridging this gap by clarifying what precisely
these features are and providing an extension to GHC that disallows
them\footnote{\url{http://hackage.haskell.org/trac/ghc/wiki/SafeHaskell}}. 
%
}

Morgenstern et al.~\cite{Morgenstern:2010} encoded an
authorization- and IFC-aware programming language in Agda.
Their encoding, however, does not consider computations with side-effects. 
%
More closely related, Devriese and Piessens~\cite{Devriese:2011} used monad
transformers and parametrized monads~\cite{Atkey06parameterisednotions} to
enforce non-interference, both dynamically and statically.
However, their work focuses on modularity (separating IFC enforcement from
underlying user API), using type-class level tricks that make it difficult
to understand errors triggered by insecurities.
Moreover, compared to our work, where programmers write standard Haskell code, 
their work requires one to firstly encode programs as values of a specific type.


\cut{
The notion of clearance originates from military settings, where it
predates the existence of computers. 
}
Compared to other language-based works, LIO uses the notion of clearance.
The work of Bell and La~Padula~\cite{bell:bell-lapadula} formalized clearance as a bound on
the current label of a particular users' processes.  In the 1980s,
clearance became a requirement for high-assurance secure systems
purchased by the US Department of Defense~\cite{Orange}.  More
recently, HiStar~\cite{zeldovich:histar} re-cast clearance as a bound
on the label of any resource created by the process (where raising a
process's label is but one means of creating a something with a higher
label).  We adopt HiStar's more stringent notion of clearance, which
prevents software from copying data it cannot read and facilitates
bounding the time during which possibly untrustworthy software can
exploit covert channels.

Simultaneously to this work, Hedin and Sabelfeld have recently published a dynamic information-flow monitor 
for a core part of Javascript which handles exceptions \cite{Hedin:Sabelfeld:CSF12}. 
Their approach needs to explicitly 
mark in the code (through non-standard constructors) which exceptions are thrown under a secret branch. Our approach, 
in contrast, simple raises an exception labeled with the current label. 


